FilterPrompt: A Simple yet Efficient Approach to Guide Image Appearance Transfer in Diffusion Models

In controllable generation tasks, flexibly manipulating the generated images to attain a desired appearance or structure based on a single input image cue remains a critical and longstanding challenge. Achieving this requires the effective decoupling of key attributes within the input image data to achieve representations accurately. Previous works have concentrated predominantly on disentangling image attributes within feature space. However, the complex distribution present in real-world data often makes the application of such decoupling algorithms to other datasets challenging. Moreover, the granularity of control over feature encoding frequently fails to meet specific task requirements. Upon scrutinizing the characteristics of various generative models, we have observed that the input sensitivity and dynamic evolution properties of the diffusion model can be effectively fused with the explicit decomposition operation in pixel space. This allows the operation that we design and use in pixel space to achieve the desired control effect on the specific representation in the generated results. Therefore, we propose FilterPrompt, an approach to enhance the effect of controllable generation. It can be universally applied to any diffusion model, allowing users to adjust the representation of specific image features in accordance with task requirements, thereby facilitating more precise and controllable generation outcomes. In particular, our designed experiments demonstrate that the FilterPrompt optimizes feature correlation, mitigates content conflicts during the generation process, and enhances the effect of controllable generation.

==> sup_result.tex <==
%More experimental results on animal appearance transfer
\begin{figure*}[b]
    \centering
    \vspace{-6mm}
    \includegraphics[width=0.9\textwidth]{illustrations/figure/FilterPrpmpt_result.pdf}
    \caption{\textbf{More experimental results on animal appearance transfer.} Compared with the baseline, we can retain more structural details, have a more accurate appearance color migration effect than IP-Adapter, and have higher imaging quality than cross-image attention.
    }
    \label{fig:sup_result}
    \vspace{-6mm}
    %\vspace{-2.0em}
\end{figure*}
